Electronic Instrumentations for High Energy Particle Physics and Neutrino Physics

The present dissertation describes design, qualification and operation of several electronic instrumentations for High Energy Particle Physics experiments (LHCb) and Neutrino Physics experiments (CUORE and CUPID). Starting from 2019, the LHCb experiment at the LHC accelerator will be upgraded to operate at higher luminosity and several of its detectors will be redesigned. The RICH detector will require a completely new optoelectronic readout system. The development of such system has already reached an advanced phase, and several tests at particle beam facilities allowed to qualify the performance of the entire system. In order to achieve a higher stability and a better power supply regulation for the frontend chip, a rad-hard low dropout linear regulator, named ALDO, has been developed. Design strategies, performance tests and results from the irradiation campaign are presented. In the Neutrino Physics field, large scale bolometric detectors, like those adopted by CUORE and its future upgrade CUPID, offer unique opportunities for the study of neutrinoless double beta decay. Their operation requires particular strategies in the readout instrumentation, which is described here in its entirety. The qualification and optimization of the working parameters as well as the integration of the system in the experimental area are also thoroughly discussed,together with the latest upgrades of two electronic subsystems for the future CUPID experiment

==> 99_Backmatter/Thanks.tex <==

\chapter*{Ringraziamenti}
\thispagestyle{empty}

...
